Exotic aromatic B-series for the study of long time integrators for a class of ergodic SDEs

We introduce a new algebraic framework based on a modification (called exotic) of aromatic Butcher-series for the systematic study of the accuracy of numerical integrators for the invariant measure of a class of ergodic stochastic differential equations (SDEs) with additive noise. The proposed analysis covers Runge-Kutta type schemes including the cases of partitioned methods and postprocessed methods. We also show that the introduced exotic aromatic B-series satisfy an isometric equivariance property.

==> Sections/Isometric_equivariance.tex <==
\label{section:isometric_equivariance}
In this section, we consider exotic aromatic rooted forests $\gamma$ where the differential associated to the root is $f$ as first defined in Section \ref{section:eat}. As the function $f$ is no longer fixed, we denote the associated differential $F(\gamma)(f)$. Also we adapt the definition of exotic aromatic B-series to this change.
First we add a new tree: the empty tree $\varnothing$.
$F$ is then extended on $\EE\AA\TT_g\cup\{\varnothing\}$ by $F(\varnothing)(f)=\Id_{\R^d}$.
Then, for a function $a:\EE\AA\TT\cup\{\varnothing\}\rightarrow \R$, the associated exotic aromatic B-series is
$$B(a)(f)=\sum_{\gamma \in \EE\AA\TT\cup\{\varnothing\}} a(\gamma) F(\gamma)(f).$$
We study (exotic) aromatic B-series $B(a)$ with $a(\varnothing)=1$. We call these (exotic) aromatic B-series methods.
Let $G$ be a subgroup of $\GL_d(\R)\ltimes \R^d$, the action of an element $(A,b)\in G$ on $\R^d$ is
$$(A,b).(x):=Ax+b,$$
and the action on a vector field $f:\R^d \to \R^d$ is
$$((A,b)*f)(x):=Af(A^{-1}(x-b)).$$
We simplify the notation by writing $A*f:=(A,0)*f$.
We recall the definition of equivariance from \cite{MuntheKaas16abs}. The property of equivariance means the method is unchanged by an affine coordinate transformation.

\begin{definition}
Let $\Phi$ be a differential operator and $G$ a subgroup of $\GL_d(\R)\ltimes \R^d$, then $\Phi$ is $G$-equivariant if
$$\forall (A,b)\in G, \forall f\in \CC^\infty(\R^d,\R^d), \Phi((A,b)*f)=(A,b)\circ\Phi(f)\circ (A,b)^{-1}.$$
In particular, $\Phi$ is said affine equivariant if $G=\GL_d(\R)\ltimes \R^d$ and isometric equivariant if $G=\Or_d(\R)\ltimes \R^d$.
\end{definition}

We say that a map $\varphi\in \CC^\infty(\CC^\infty(\R^d,\R^d),\CC^\infty(\R^d,\R^d))$ is local if for all smooth $f$, the support of $\varphi(f)$ is included in the support of $f$. The locality of exotic aromatic B-series is straightforward.
Munthe-Kaas and Verdier showed in \cite{MuntheKaas16abs} that the only affine equivariant and local numerical integrators are the aromatic B-series methods.
In this section, we show the exotic aromatic B-series methods are isometric equivariant.
\begin{remark}
It would be interesting to know if the isometric equivariance and locality of a map yields that it can be expanded as an exotic aromatic B-series.
\end{remark}

We notice this first result: if $G=H\ltimes \R^d$, $B(a)$ a B-series method with $B(a)(f)=\Id+\Phi(f)$,then $B(a)$ is $G$-equivariant if and only if $\Phi$ is $H\times\{0\}$-equivariant.
Thus, we call $H$-equivariance the $H\times \{0\}$-equivariance for simplicity.

\begin{ex*}
Let us show the Laplacian operator is $\Or_d(\R)$-equivariant and not $\GL_d(\R)$-equivariant.
We take $A=(a_{i,j})\in \GL_d(\R)$, denote $B=(b_{i,j})=A^{-1}$ its inverse and choose $f$ a smooth function, then
$$\frac{\partial (A*f)_j}{\partial x_i}(x)=\sum_{k,l} a_{j,k}b_{l,i}\frac{\partial f_k}{\partial x_l}(A^{-1}x).$$
And the Laplacian is given by
$$\Delta (A*f)_j(x)=\sum_{k,l,m} a_{j,k} \left(\sum_i b_{l,i}b_{m,i}\right)\frac{\partial^2f_k}{\partial x_l\partial x_m}(A^{-1}x).$$
On the other side,
$$(A\Delta f(A^{-1}x))_j=\sum_{k,l} a_{j,k}\frac{\partial^2f_k}{\partial x_l^2}(A^{-1}x).$$
We freeze $A$ and we choose $f^{(u,v,k_0)}_k(x)=x_u x_v \delta_{k,k_0}$ for $u,v,k_0$ in $\{1,\dots,d\}$ then if $\Delta$ is $\GL_d(\R)$-equivariant, we must have the following equality
$$\forall j,\forall x, \Delta (A*f^{(u,v,k_0)})_j(x)=a_{j,k_0}\sum_i b_{u,i} b_{v,i}=a_{j,k_0}\delta_{u,v}=(A\Delta f^{(u,v,k_0)}(A^{-1}x))_j.$$
As $a_{j,k_0}$ can not be null for every $j$ because $A\in \GL_d(\R)$, we find $\sum_i b_{u,i} b_{v,i}=\delta_{u,v}$ and thus $A$ must be in $\Or_d(\R)$.
We check quickly that if $A\in \Or_d(\R)$ then $\Delta (A*f)_j(x)=(A\Delta f(A^{-1}x))_j$.
Thus the Laplacian operator is $\Or_d(\R)$-equivariant, but is not $\GL_d(\R)$-equivariant.
\end{ex*}

This example hints us that the right group $G$ for equivariance of exotic aromatic B-series is $\Or_d(\R)\ltimes \R^d$ as shown in the following theorem.

\begin{theorem}
\label{theorem:equivariance}
Let $B$ be an exotic aromatic B-series method $B(a)$ (with $a(\varnothing)=1$), then $B$ is isometric equivariant.
\end{theorem}

\moda{The idea of the proof is a generalization of the one we did for the affine equivariance of the Laplacian operator. In the spirit of the result \cite[Prop.\ts 2.1]{MuntheKaas16abs} for affine equivariant B-series, we first find and simplify patterns linked with affine equivariance by bringing together sums concerning pairs of nodes linked by edges. Then we bring together the sums concerning pairs of nodes linked by lianas.}
%The detailed proof is in Appendix \ref{appendix:isometric_equivariance}.



==> Sections/general_additive_noise.tex <==
In this section, we generalize the previous work to the research of numerical integrators for the invariant measure for the SDE
\begin{equation}
\label{sde0}
dX=f(X)dt+\Sigma^{1/2}dW,
\end{equation}
where $\Sigma$ is a symmetric definite positive matrix.
By an orthogonal change of variable, we can suppose $\Sigma$ is a diagonal matrix. We denote $\sigma_i^2$ its diagonal coefficients.





\moda{TO BE COMPLETED : ajouter références, adapter hypothèses et formalisme à ce cas plus général.}




 
We can adapt the previous formalism in the following ways.
\begin{itemize}
\item In all the proposed numerical integrators, we replace $\xi$ by $\Sigma^{1/2}\xi$.
\item Definition \ref{elementary_differential} is upgraded with the following elementary differential formula : if $\gamma \in \EE\AA\TT_g$, then
$$F(\gamma)(f,\phi,\xi)=\sum_{i_{v_1},...,i_{v_m}=1}^d \sum_{j_{l_1},...,j_{l_s}=1}^d \left(\prod_{v\in V^0} \partial_{I_{\pi(v)}} \partial_{J_{\Gamma(v)}} f_{i_v}\right)
\left(\prod_{v\in V_g} \sigma_{i_v} \xi_{i_v}\right) \partial_{I_{\pi(r)}} \partial_{J_{\Gamma(r)}} \phi.$$
\item Theorem \ref{Theorem:Forest_expectation} is still true. To extend the proof, we notice $F(\gamma)(\phi)$ is a $2n$-multilinear form $B_{\gamma,\phi}$ evaluated in $(\Sigma^{1/2}\xi,...,\Sigma^{1/2}\xi)$, then we consider $\widetilde{B}_{\gamma,\phi}(x_1,...,x_{2n}) = B_{\gamma,\phi}(\Sigma^{1/2}x_1,...,\Sigma^{1/2}x_{2n})$. We can apply Lemma \ref{Lemma:Forest_expectation} to $\widetilde{B}_{\gamma,\phi}$, and it gives the desired result by simple calculation.
\item The integration by parts of Theorem \ref{Theorem:IPP} is adapted straightforwardly.
\end{itemize}
But, under Assumption \ref{Assumption:f_gradient}, we can not in general adapt the simplification rule (Proposition \ref{Proposition:Simplification_rule}). In order to study the numerical integrators, one must keep the aromatic roots in the computations, thus getting numerous new order conditions.
Under the following assumption, we can adapt Proposition \ref{Proposition:Simplification_rule}.

\begin{ass}
\label{Assumption:f_gradient_V_non_couple}
$f$ is a globally Lipschitz gradient, i.e.\ there exists a $C^\infty$ potential $V :\R^d\rightarrow \R$ such that $f(x)=-\nabla V(x)$ is globally Lipschitz and
there exist $C_1>0$ and $C_2$ such that for all $x\in\R^d$,
$$
V(x) \geq C_1 x^T x - C_2.
$$
In addition, the potential $V$ is of the form
$$V(x_1,...,x_d)=V_1(x_1)+...+V_d(x_d).$$
\end{ass}

Under this assumption, $\rho_\infty(x)=\frac{1}{Z}\prod_j \exp\left(-\frac{2V_j(x_j)}{\sigma_j^2}\right)$ and $\nabla g=2\Sigma^{-1} f$.

\begin{proposition}[New Simplification Rule]
\label{Proposition:New_simplification_rule}
Under Assumption \ref{Assumption:f_gradient_V_non_couple}, the two forest patterns gathered in each of the following pairs represent the same differential :
\begin{enumerate}
\item $\includegraphics[scale=0.5]{Other_trees/simplificationrule5.eps}$ and $\frac{2}{\sigma^2} \includegraphics[scale=0.5]{Other_trees/simplificationrule6.eps}$,
\item $\gtree 1 1 1 1$ and $\frac{2}{\sigma^2} \etree 1 2 0 1$.
\end{enumerate}
The node B can also be replaced.
\end{proposition}

Then all the consistency and order 2 conditions of theorems of Sections \ref{section:formal_ipp}, \ref{section:Runge_Kutta}, \ref{postprocessed integrators} and \ref{section:partitioned_methods} still hold under Assumption \ref{Assumption:f_gradient_V_non_couple} and by replacing $\xi$ by $\Sigma^{1/2}\xi$ in the numerical methods.
But, as the differentials associated to $\etree 3 1 1 4$ and $\etree 3 2 1 2$ can no longer be identified, the conditions for order 3 are modified and there is a extra condition associated to the tree $\etree 3 2 1 2$.
The interested reader can ask the authors for the details of these new conditions.


